Data-Driven Cellular Network Selector for Vehicle Teleoperations

Remote control of robotic systems, also known as teleoperation, is crucial for the development of autonomous vehicle (AV) technology. It allows a remote operator to view live video from AVs and, in some cases, to make real-time decisions. The effectiveness of video-based teleoperation systems is heavily influenced by the quality of the cellular network and, in particular, its packet loss rate and latency. To optimize these parameters, an AV can be connected to multiple cellular networks and determine in real time over which cellular network each video packet will be transmitted. We present an algorithm, called Active Network Selector (ANS), which uses a time series machine learning approach for solving this problem. We compare ANS to a baseline non-learning algorithm, which is used today in commercial systems, and show that ANS performs much better, with respect to both packet loss and packet latency.

==> sections/old.tex <==
\textcolor{red}{The runtime complexity of ANS is the runtime of the two ML models used for the prediction plus a constant additional overhead of code steps. We can treat the computation of each layer's operations as a constant time relative to our specified input size of $9x64$, where nine represents the number of feature channels (our 9-feature model) and 64 represents the window length. For the convolutional layers, the complexity is $O(C_{in} \cdot C_{out} \cdot K \cdot L)$ where $C_{in}$ and $C_{out}$ represent the number of input and output channels, respectively, $K$ is the kernel size, and $L$ is the window length. For the LSTM layers, the complexity is derived from the formula $O(T\cdot 4 \cdot (D\cdot H + H^{2}))$, with $T$ representing the number of time steps (64), $D$ is the input dimension from our last convolutional later (128), and $H$ is the hidden size (128). For the fully connected layers, it involves matrix multiplications, which, due to fixed input and output dimensions, add further to the constant-time assertion. Under the assumption that the input dimensions and model architecture do not change, the computational complexity of this neural network can be considered constant, thus $O(1)$.}
